E(3)-Equivariant Mesh Neural Networks

Triangular meshes are widely used to represent three-dimensional objects. As a result, many recent works have address the need for geometric deep learning on 3D mesh. However, we observe that the complexities in many of these architectures does not translate to practical performance, and simple deep models for geometric graphs are competitive in practice. Motivated by this observation, we minimally extend the update equations of E(n)-Equivariant Graph Neural Networks (EGNNs) (Satorras et al., 2021) to incorporate mesh face information, and further improve it to account for long-range interactions through hierarchy. The resulting architecture, Equivariant Mesh Neural Network (EMNN), outperforms other, more complicated equivariant methods on mesh tasks, with a fast run-time and no expensive pre-processing. Our implementation is available at https://github.com/HySonLab/EquiMesh

==> old/1.introduction.tex <==
The unprecedented developments in 3D geometric deep learning have demonstrated remarkable performance in a wide range of tasks in computer graphics and vision. Apart from several alternative representations used for three-dimensional objects, such as voxels and point clouds, triangular meshes not only allow effectively capturing large and simple surfaces but also offer a flexible way for rendering and reconstruction at high resolutions \cite{10.1145/3355089.3356488}. More specifically, meshes consist of both geometric and topological components, meaning that in addition to encoding rich semantic information via the geometric aspects of their underlying surfaces, triangular meshes also provide connectivity information between their vertices, edges, and faces \cite{10.5555/863276}. The implication of this is that methods working on mesh data should involve shape identity and structure-aware understanding in learning the representations of 3D meshes, resulting in superior abstraction from low-level to high-level elements.\\

Geometry plays a key role in creating a deep network for mesh data. In particular, the proposed network should be equivariant geometric transformations, such as  translations and rotations. While some existing methods are do not have invariance or equivariance guarantees \cite{laplacian2mesh, meshmlp}, many existing methods use symmetry by relying on invariants of geometric transformations as their input and, therefore, are not as expressive as equivariant architectures. \siamak{are we sure meshmlp and Laplacian are not invariant?}
For example, \cite{egnn-sc} uses invariant features such as volumes, angles, and distances in processing simplicial complexes, which include mesh data. 

Moreover, in contrast to graph neural networks, the additional structure, due to the triangular faces, should be used in learning with mesh. While graph-based methods have been successfully applied to the mesh, they do not benefit from the fine-grained structure of the mesh \cite{graph_13, graph_14, graph_15,graph_16}. Moreover, equivariant neural networks built upon the message-passing scheme underperform on large mesh data due to over-smoothing and over-squashing, which is problematic in the presence of long-range interactions. \siamak{do we see this in experiments? citation?} 

The final factor in our desiderata is simplicity. While several frameworks, in particular convolution \cite{gemcnn, meshnet, meshcnn, cnn30, cnn31, cnn32, cnn33} and attention-based \cite{eman} approaches, satisfy the above requirements, they are often more complex, both conceptually and practically. 

In this work, we address these issues by \emph{minimally} extending the widely used $E(n)$-equivariant graph neural networks (EGNN) to adapt them to mesh data. The resulting method, called Equivariant Mesh Neural Network (EMNN), is a simple message-passing method that proves both efficient and effective in comparison to all prior work. To better model long-range interactions, we further equip EMNN with hierarchy by enabling interaction between equivariant and invariant features at multiple scales.

Similar to EGNN the proposed method maintains and updates invariant scalars and equivariant vectors in each layer. However, these invariants now incorporate the face geometry of the mesh, using updates that effectively calculate surface area and normals. Since surface normals are not equivariant to reflection, they break the reflection symmetry of EGNN, producing equivariance to the Special Euclidean group. We believe this is an important feature for processing mesh data since it discriminates between the inside and outside of the mesh. \cref{table:symmetry} contrasts the invariance and equivariance properties of existing architectures with our EMNN.\siamak{Ideally, all methods for mesh that we cite should be listed in this table}


\begin{table}[h!]
\begin{center}
\caption{Invariance and equivariance property of mesh networks. }\label{table:symmetry}
\vspace{5pt}
\begin{tabular}{l c c c c c c c c}
\toprule
Method & \multicolumn{2}{c}{Rotation} & \multicolumn{2}{c}{Translation} & \multicolumn{2}{c}{Reflection} & \multicolumn{2}{c}{Scale} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& \rotatebox{90}{invariant} & \rotatebox{90}{equivariant} & \rotatebox{90}{invariant} & \rotatebox{90}{equivariant} & \rotatebox{90}{invariant} & \rotatebox{90}{equivariant} & \rotatebox{90}{invariant} & \rotatebox{90}{equivariant} \\
\midrule
GWCNN \cite{gwcnn} & \cmark & \xmark & \cmark & & ? & & - & \\ 
MeshCNN \cite{meshcnn} & \cmark & \xmark & \cmark & & ? & & \cmark & \\
PD-MeshNet \cite{Milano20NeurIPS-PDMeshNet} & \cmark & \xmark & \cmark & & ? & & \cmark & \\
MeshWalker\cite{lahav2020meshwalker} & \cmark & \xmark & \cmark & & ? & & \cmark & \\
SubdivNet \cite{DBLP:journals/tog/HuLGCHMM22} & \xmark & \xmark & \xmark & & ? & & \cmark & \\
HodgeNet \cite{smirnov2021hodgenet} & \cmark & \xmark & \cmark & & ? & & \cmark & \\
DiffusionNet\cite{diffusionnet} & \cmark & \xmark & \cmark & & ? & & \cmark & \\
Laplacian2Mesh \cite{laplacian2mesh} & \xmark & \xmark & \xmark & & ? & & \xmark & \\
Mesh-MLP \cite{meshmlp} & \xmark & \xmark & \xmark & \xmark & ? & & \xmark & \\
\midrule
GEM-CNN \cite{gemcnn} \\
EMAN \cite{eman} \\
\midrule
EMNN (ours) & \cmark & & \cmark & & ? & & \cmark & \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


% \begin{table}[h!]
% \begin{center}
% \caption{Robust to transformations - Rotation, Translation, and Scale.}
% \vspace{5pt}
% \begin{tabular}{l c c c}
% \toprule
% Method & Rotation & Translation & Scale \\
% \midrule
% GWCNN \cite{gwcnn} & \cmark & \cmark & - \\ %  encode using physics based on distance matrix ???
% MeshCNN \cite{meshcnn} & \cmark & \cmark & \cmark\\
% PD-MeshNet \cite{Milano20NeurIPS-PDMeshNet} & \cmark  & \cmark & \cmark \\ % only dihedral angles
% MeshWalker\cite{lahav2020meshwalker} & \cmark & \cmark & \cmark \\ % random walk
% SubdivNet \cite{DBLP:journals/tog/HuLGCHMM22} & \xmark & \xmark & \cmark \\ % use face center
% HodgeNet \cite{smirnov2021hodgenet} & \cmark & \cmark & \cmark \\ % hks vs invariant features
% DiffusionNet\cite{diffusionnet} & \cmark & \cmark & \cmark \\ % Laplace & mass matrix and spatial gradient matrix (invariant to the choice of local tangent basis)
% Laplacian2Mesh \cite{laplacian2mesh} & \xmark & \xmark & \xmark \\
% Mesh-MLP \cite{meshmlp} & \xmark & \xmark & \xmark \\
% \midrule
% MeshEGNN (ours) & \cmark & \cmark & \cmark\\
% MeshEGNN + MC (ours) & \cmark & \cmark & \cmark\\
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}


\siamak{Ok, I rewrote the intro and put more focus on simplicity. Invariance to scale, and multi-channel are not key, since the first one is only using preprocessing, and the latter is not new. Also for consistency the name is changed to EMNN.}



==> old/2.related_works.tex <==
% {
% \color{blue}
% Outline:
% \begin{itemize}
%     \item P1: Graph based mesh methods
%     \item P2: Equivariant methods
%     \item P3: Hierarchy
%     \item P4: Multi-channel
% \end{itemize}
% }

\siamak{Let's improve the organization and classification of related methods in this section, ideally make them coherent with the introduction. I'll skip for now.}

\paragraph{Graph-based Deep Learning for Mesh} Previous graph-based models redesign GCNs to work on meshes by using a shared isotropic kernel to the mesh vertices and its k-ring neighbours \cite{graph_13, graph_14,graph_15}. Due to the invariance of their message-passing formulas to the surface position, the local variations in the regularity and isotropy of mesh elements may not be captured.\siamak{not sure what the sentence means. clarify?} \cite{graph_16} partially resolve this limitation by adding the learnable weights between the targets and its neighbour when updating the feature, which is similar to the attention mechanism. Noticeably, all aforementioned methods pool the meshes based on a generic graph clustering algorithm. Later methods such as \cite{graph_26, graph_28} propose a pooling that relies on the geometry of the mesh.
%\paragraph{Equivariance on graphs and manifolds} Equivariance on graphs and manifolds has been studied from numerous perspectives. \cite{eman_18, eman_19a} propose novel gauge equivariant convolution techniques on manifolds such as spheres and platonic solids. \cite{egnn} propose $E(n)$ -equivariant graph neural network models, which are applied to equivariant normalizing flows by \cite{kohler2020equivariant}. Moreover, \cite{gemcnn} point out a relation between different types of equivariances: their gauge equivariant model is also equivariant to the group of isometries of the given mesh. The equivariance with respect to this group of isometries has been extensively studied by \cite{weiler2021coordinate} and \cite{cohen2021thesis}. In contrast, our work focuses on equivariance with respect to gauge transformations and global transformations of R3. (Copied from EMAN)
\paragraph{Mesh as Manifold}
By interpreting the mesh as a discretization of a manifold, some methods interpret a node's neighbourhood as a 2-dimensional surface, applying a convolutional filter over the node and its neighbours.
Previous works that have applied convolutions to manifolds include  \cite{weiler2021coordinate, eman_18, eman_19a}.
Such methods either use isotropic filters, such as in, \cite{} \textcolor{blue}{cite} or have enforced gauge equivariance: that is, indifference to the choice of the local coordinates in which the filters are applied. This can be accomplished by using kernels derived from representations of 2-dimensional rotations and mapping between different coordinate frames at different nodes using parallel transport. Examples of this class of neural networks include \cite{eman} and \cite{gemcnn}.


\paragraph{Geometric Graph Learning for Mesh}
Motivated by tasks in chemistry and physical sciences, many deep learning methods have been designed to act on geometric graphs: that is, graphs whose nodes have coordinates.
Such methods are therefore invariant or equivariant to the Euclidean group E(n) of rotations, translation, and reflections in $n$ dimensional space.
Popular methods include those that extend message passing to use invariant features (e.g. distances and angles) such as \cite{schutt2018schnet} and \cite{gasteiger2020directional}.
Other approaches use higher-order tensor representations of rotations to equivariantly encode geometric features of nodes, such as \cite{thomas2018tensor} and \cite{brandstetter2021geometric}.
One prominent method that combines features of both these approaches is the E(n)-equivariant Graph Neural Network (E(n)-EGNN) \citep{egnn}, which computes invariant features over edges and uses them to update equivariant coordinates for each node.  
% Recently, \cite{levy2023using} found that extending E(n)-EGNN to encode multiple equivariant vectors per node resulted in improved performance across tasks.


%\paragraph{Multi channels}
%to achieve high expressivity \cite{mc-2022}. Prior works, however, show that one can achieve satisfactory modeling performance without requiring higher-order representations. One such example is the Vector Neurons \cite{mc-2021} model, which can be seen as an equivariant multilayer perceptron with order-1 vector features. This architecture also leverages the fact that the number of vector channels (neurons) in each layer can be arbitrary to increase expressivity. --- (Copy from multi channel paper need to rewrite)
% \paragraph{Pooling} 
% \begin{itemize}
%     \item graph based 
%     \item mesh based
% \end{itemize}


==> old/3.background.tex <==
In this section, we provide background information on mesh representations and $E(n)$ equivariant graph neural networks, which are essential for understanding our method.

\subsection{Mesh Representation}
\label{sec:mesh}
Polygon mesh, which is a collection of vertices and polygons, is an alternative to point clouds and voxels-based representations of 3D objects. In this work, we focus on triangle meshes. Mathematically, a triangle mesh is defined as a triplet $\set{M} = (\set{P},\set{E},\set{F})$, where $\set{P}$ is a set of points in 3D space, called vertices, $\set{E}$ is the edge set, where each edge is a pair of vertices, and $\set{F}$ is a set of triangle faces, where each face is a triplet of nodes. We denote $n = \lvert \set{P} \rvert$, the number of vertices in the mesh. 

The mesh $\set{M}$ should additionally satisfy the following constraints: every edge belongs to either one or two triangles.
The intersection of two distinct triangles is either an edge, a vertex, or empty. The mesh is manifold, which means that the local topology around each vertex resembles a disk. This implies that the triangles are consistently oriented and that there are no holes in the mesh. Triangle meshes are easy to store and render and can be used to represent a wide variety of objects \cite{rogers1986procedural}. 
 
% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=0.8\linewidth]{iclr2024/visualization/mesh.png}
%   \caption{\label{fig:update} Mesh \siamak{This one is not a very useful figure. Let's drop?}}
% \end{figure}
\paragraph{Geometric Feature on Meshes}  Mesh vertices, edges and faces of the mesh can have additional attributes. For geometric learning, we find the following attributes relevant. Each point $p \in \set{P}$ is associated with its 3D coordinate vector $x_p \in \R ^ 3$. Meanwhile, a face $f \in \set{F}$ can have scalar and vector attributes corresponding to the area and normal vector, denoted by ${a}_f$ and $n_f$ respectively. Considering a triangle face  $f = (p_1, p_2, p_3)$, the normal vector and the area are given by $n_f = (x_{p_2} - x_{p_1}) \times (x_{p_3} - x_{p_1})$ and $a_f = \frac{\lvert \lvert n_f \rvert \rvert}{2}$ respectively. Furthermore, the normal vector (area) associated with each point $p \in \set{P}$ can be defined via a weighted sum of normal vectors (area) of its adjacent faces:
\begin{equation}
    n_p := \frac{\sum_{f \ni p} a_{f} n_{f_i}}{\lvert \lvert \sum_{f \ni p} a_{f} n_{f_i} \rvert \rvert}, \quad a_p := \frac{\sum_{f \ni p} a_f}{|\{f \mid p \in f\}|} \label{eq_0},
\end{equation}
where $ f \ni p \equiv  \{f \mid p \in f\}$ denotes faces that contain $p$. $n_p \in \R ^ 3$ and $a_p \in \R$ can act as SE(3) - equivariant and invariant features for point $p$. In particular, note that $n_p$ is not equivariant to reflection; the normal to the surface of a triangle reflected by a 2D plane in 3D space is not the reflection of the original normal vector. 

% and we denote $n = \lvert \mathcal{P} \rvert$. Each point $v_i$ in $\mathcal{P}$ is associated with its three-dimensional coordinate $x_i \in \R ^ 3$. Given the three mentioned primary components of $\mathcal{M}$, we can compute other equivariant features for each node $v_i$, such as normal vectors $\mathbf{n}_i \in \R ^ 3$, and stacking $m$ the equivariant features of $v_i$ result in multi-channel equivariant feature $X_i \in \R ^ {3 \times m}$. 


\subsection{Equivariant Graph Neural Networks}
\label{egnn}

The original $E(n)$- Equivariant Graph Neural Networks (EGNNs) extend the message-passing framework operating on graphs to geometric graphs involving their vertices' spatial information. In particular, a geometric graph is defined as $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with two main components: vertices $v_i \in \mathcal{V}$ and edges $e_{ij} \in \mathcal{E}$. Each vertex $v_i$ is associated with scalar invariant features $h_i \in \R ^ d$ and $n$-dimensional equivariant coordinates $x_i \in \R ^ n$. To make the messages invariant to $E(n)$ transformations, each EGNN's layer takes into account the relative Euclidean distance between two coordinates $x_i$ and $x_j$ as the input for its message update function $\phi_e$: 
\begin{align}
    x_{ij} &= x_i - x_j, \label{eq_1} \\
    m_{ij} &= \phi_e(h_i^l, h_j^l, \|x_{ij}\| ^ 2, e_{ij}), \label{eq_2} \\
    m_i &= \sum_{j \in \epsilon(i)} m_{ij}. \label{eq_3} 
\end{align}
Then, the coordinate $x_i$ and scalar feature $h_i$ at the layer $l+1$ are updated by the following equations:
\begin{align}
    %x_i^l &= \sum_{j \in \epsilon(i)} x_{ij} \phi_x (m_{ij}), \label{eq_4} \\
    x_i ^ {l+1} &= x_i ^ {l} + \alpha  \sum_{j \in \epsilon(i)} x_{ij} \phi_x (m_{ij}), \\ 
    h_i ^ {l+1} &= \phi_h(h_i ^ {l}, m_i) \label{eq_5}, 
\end{align}
Here $h_i^l$, $x_i^l$, $e_{ij}$ denotes node embeddings, coordinate embeddings, and edge features at layer $l$, respectively. Additionally, $\phi_e : \R^{d_h + d_h+1+d_e} \to \R^d$, $\phi_x : \R^d \to \R$, and $\phi_h : \R^{d_h+d} \to \R^{d_h}$ are multi-layer perceptrons (MLPs) and $\epsilon(i)$ denotes the set of neighbours of node $i$. EGNNs can preserve equivariance to translations, rotations, and permutations as the networks are built upon the message-passing framework and use relative squared distances in the message functions.

\siamak{I don't think we need a separate intro to multi-channel. When proposing our method, we can say following levy et al, we use multiple vector channels for better expressivity.}
\paragraph{Multi-Channel Equivariant Graph Neural Networks}
Following \cite{levy2023using}, EGNNs can be extended to include multiple vector channels by replacing $x_i$ with the matrix $X_i \in \R^{3 \times m}$, where $m$ is the number of vector channels. More specifically, Equations (\ref{eq_1}, \ref{eq_2}, \ref{eq_3}) are modified to adapt to the multi-channel setting:
\begin{align}
    X_{ij} &= X_i - X_j, \\
    m_{ij} &= \phi_e(h_i^l, h_j^l, \lvert \lvert X_{ij} \rvert \rvert _ c ^ 2, e_{ij}), \\
    X^{l+1}_i &= X^l_{i} + \alpha\sum_{j \in \epsilon(i)} X^l_{ij}\phi_x (m_{ij} \label{eq_9}), 
\end{align}
for MLPs $\phi_e: \R^{d_h+d_h+m+d_e} \to \R^d$
and $\phi_x:\R^d \to \R ^ {m \times m ^ \prime}$, where $m^\prime$ is the output channel dimension. $\lvert \lvert X_{ij} \rvert \rvert _ c$ denotes the Euclidean norm applied across each channel. 
%We set m = 1 for the first and last layer to use a single vector for each node’s inputs and outputs.
%The modification to EGNN does not affect the equivariance properties of the architecture since the Euclidean and permutation groups do not act over the channels' dimensions.

% {\color{blue}{More explanation} ???} \par
% The multi-channel version of EGNNs is naturally extended by replacing $\mathbf{x_i}$ with the matrix $\mathbf{X_i} \in \R^{3 \times m}$, where $m$ is the number of vector channels. Consequently, the Multi-Channel $E(n)$ - Equivariant Graph Neural Network (MC-EGNN) is rewritten as: 
% \begin{align*}
%     X_{ij} &= X_i - X_j, \\
%     m_{ij}^l &= \phi_e(h_i^l, h_j^l, X_{ij}, \mathbf{a}_{ij}), \\
%     X^{l+1}_i &= X^l_{i} + \alpha\sum_{j \in \epsilon(i)} \phi_x (m_{ij}). 
% \end


 %%%%%%%%%%%% Comment %%%%%%%%%%%%
% The original $E(n)$- Equivariant Graph Neural Networks (EGNNs) applies on a geometric graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with 2 main components: vertices $v_i \in \mathcal{V}$ and edges $e_{ij} \in \mathcal{E}$


% \section{Method}

% \subsection{Multi-Channel Mesh $E(n)$ - Equivariant Graph Neural Network (MC-MeshEGNN)}
% We extend the formulation of multi-channel EGNNs as described in Section \ref{mc_egnn} to Triangle meshes, which are two-ordered. In particular, we 

% A typical mesh $\mathcal{M} = (\mathcal{P}, \mathcal{E}, \mathcal{F})$ combine 3 main components: points $\mathcal{P} \in \R^{n \times 3}$, edges $\mathcal{E} \in \R^{e \times 2}$, and faces $\mathcal{F} \in \R^{f \times 3}$. From these components, it is easy to compute other important information such as normal vectors $N \in \R^{n \times 3}$ and dihedral angles $\mathcal{A} \in \R^{f \times 3}$. In some settings, there are also pre-computed features $H \in \R^{n \times d}$. \\
% Regarding our adaptation from graph to mesh, we initially combine both $\mathcal{P}$ and $N$ into matrix of two vectors $C \in \R^{n \times 3 \times 2}$. Moreover, we also introduce new aggregation to extract information from Triangle faces called $m_{\tau(i)}$ beside the edge information $m_{\epsilon(i)}$. All the steps are formalized as follow:
% \begin{align*}
%     C &= [x, n], \\
%     C_{ij} &= C_i - C_j, \\
%     m_{ij}^l &= \phi_e(h_i^l, h_j^l, \|C_{ij}\|^2_c, a_{ij}), \\
%     m_{\epsilon(i)} &= \sum_{j \in \epsilon(i)} m_{ij}, \\
%     h_{ijk} &= \phi_M (h_i, h_j, \psi_{ij}) + \phi_M(h_j, h_k, \psi_{jk}) + \phi_M(h_k, h_i, \psi_{ik}), \\ 
%     m_{ijk} ^ {l} &= \phi_s(h_{ijk}, \frac{\|(C_j ^ {l} - C_i ^ {l}) \times (C_k^{l}- C_i^{l}) \|_2 ^ 2}{2}), \\
%     m_{\tau(i)} &= \sum_{j, k \in \tau(i)} m_{ijk}. \\ 
% \end{align*}

==> old/4.method.tex <==
This section presents our proposed Multi-channel SE(3)-Equivariant Mesh Neural Networks to learn representations of triangle meshes. Unlike other methods, our approach employs only the raw vertex coordinates and scalar features to model geometric shapes more expressively. Indeed, our approach is SE(n)-equivariant and scale-invariant.

% Consequently, the Multi-Channel $E(n)$ - Equivariant Graph Neural Network (MC-EGNN) is rewritten as:

% where:
% \begin{itemize}
%     \item $x_i^l$: position of the target point at layer $l$
%     \item $x_j^l$: absolute position of the neighbour points at layer $l$
%     \item $F_j$: features of neighbour points ($f_j^l$ is the normal vector)
% \end{itemize}
\subsection{Equivariant Message Passing on Triangle Meshes}
% \begin{align*}
%     m_{ij}^l &= \phi_e(h_i^l, h_j^l, \|x_i^l - x_j^l\|_2), \\
%     x_i ^ {l+1} &= x_i ^ {l} + C \sum_{x_j^{l} \in \mathcal{N}(x_i^{l})} (x_i^l - x_j^l) \phi_x (m_{ij}), \\ 
%     m_i &= \sum_{j \neq i} m_{ij}, \\
%     h_i ^ {l+1} &= \phi_h(h_i ^ {l}, m_i).
% \end{align*}
%Extended version (Idea from meetings)

\begin{figure}[h!]
  \centering
  \includegraphics[width=1.0\linewidth]{iclr2024/visualization/layer.png}
  \caption{\label{fig:layer} EGNN Layer}
\end{figure}

\siamak{Too many equations. Merge and simplify, similar to what we wrote in the meeting.}
We extend the original EGNNs with surface-aware invariant information on triangle meshes, which are essential in learning to represent geometric shapes. More specifically, in addition to the relative squared distances between two pairs of nodes like Equations \ref{eq_1}, we take into account areas and normal vectors of the surfaces as invariant and equivariant features, respectively. Considering a triangle face ($i$, $j$, $k$), we define a surface-aware message as:
\begin{equation}
    m_{ijk}  = \phi_s\bigg(h_i ^ {l}, h_j ^ {l} + h_k ^ {l}, \frac{\lvert \lvert (X_j ^ {l} - X_i ^ {l}) \times (X_k ^ {l}- X_i ^ {l}) \rvert \rvert_c}{2}\bigg). \label{eq_10} \\
\end{equation}
In Equation \ref{eq_10}, for each vertex $v \in (i, j, k)$, we input the surface's area and means of its two adjacent vertices $j$ and $k$ as invariant messages. Then, we aggregate the messages propagated to the vertex $i$ and update its equivariant and invariant features $X_i^{l+1}$ and $h_i^{l+1}$ at layer $(l+1)$ as follows:
% \begin{equation}
%           X_i ^ {l+1} = x_i ^ {l} + C \sum_{j \in \epsilon(i)} (X_i^l - X_j^l) \phi_x (m_{ij}) + \sum_{j,k \in \tau(i)} [(X ^ {l} _j - X_i ^ {l}) \times (X_k ^ {l} - X_i ^ {l})] \phi_t(m_{ijk}), 
% \end{equation}
\begin{align}
    m ^ e _{i} &= \sum_{j \in \epsilon(i)} m_{ij}, \label{eq_11} \\%+  \sum_{(j, k) \in \tau(i)} m_{ijk}, \label{eq_11} \\
    m ^ f_{ i} &= \sum_{(j, k) \in \tau(i)} m_{ijk}, \label{eq_12} \\
    h_i ^ {l+1} &= \phi_h(h_i ^ {l}, m ^ e _ i, m ^ f _ i), \label{eq_13} \\
    X_{i}^e &= \sum_{j \in \epsilon(i)} (X_i^l - X_j^l) \phi_x (m_{ij}),\label{eq_14} \\
    X_{i}^f &= \sum_{j,k \in \tau(i)} [(X ^ {l} _j - X_i ^ {l}) \times (X_k ^ {l} - X_i ^ {l})] \phi_t(m_{ijk}), \label{eq_15} \\
    %X_i ^ {l+1} &= \phi_v(h_i ^ l) + \alpha X_{\epsilon(i)}^{l+1} + \beta X_{\tau(i)}^{l+1}, \\
    X_i ^ {l+1} &= X_i ^ l + X ^ e _ {i} + X_{i} ^ f \label{eq_16}.
\end{align}
% \begin{align}
%     m_{\epsilon(i)} &= \sum_{j \neq i} m_{ij} +  \sum_{j \neq i, k \neq i} m_{ijk}, \label{eq_11} \\
%     m_{\tau(i)} &= \sum_{j \neq i, k \neq i} m_{ijk}, \label{eq_12} \\
%     h_i ^ {l+1} &= \phi_h(h_i ^ {l}, m_{\epsilon(i)}, m_{\tau(i)}), \\
%     X_{\epsilon(i)}^{l+1} &= \sum_{j \in \epsilon(i)} (X_i^l - X_j^l) \phi_x (m_{ij}),\label{eq_14} \\
%     X_{\tau(i)}^{l+1} &= \sum_{j,k \in \tau(i)} [(X ^ {l} _j - X_i ^ {l}) \times (X_k ^ {l} - X_i ^ {l})] \phi_t(m_{ijk}), \label{eq_15} \\
%     %X_i ^ {l+1} &= \phi_v(h_i ^ l) + \alpha X_{\epsilon(i)}^{l+1} + \beta X_{\tau(i)}^{l+1}, \\
%     X_i ^ {l+1} &= X_i ^ l + \alpha X ^ {l+1} _ {\epsilon(i)} + \beta X_{\tau(i)} ^ {l+1} \label{eq_16}.
% \end{align}
Here, we use $\epsilon(i) = \{ j | (i, j) \in \mathcal{E} \}$ and $\tau(i) = \{(j, k) | (i, j, k) \in \mathcal{F}\}$ to denote the set of all neighbours of vertex $i$ that form edges and faces with it, respectively.



In Equations \ref{eq_11} and \ref{eq_12}, $m ^ e _{i}$ and $m ^ f_i$ are two types of messages aggregated from all edges $(i, j) \in \mathcal{E}$ and faces $(i, j, k) \in \mathcal{F}$ that contain the vertex $i$ at their boundaries. The scalar invariant feature $h_i ^ {l+1}$ is updated by a function $\phi_h: \R ^ {d_h + d + d} \mapsto \R ^ {d_h}$ that takes the $m ^ e _ i$ and $m ^ f_{i}$ with the previous $h_i ^ {l}$ at layer $l$ as inputs. Indeed, the update function in Equation \ref{eq_13} is the extension version of Equation \ref{eq_5} in which we consider the invariant features of surfaces. Similarly, the multi-channel equivariant feature of each vertex $X_i$ is computed using two weighted sums: (1) a weighted sum of relative differences $(X_i - X_j)_{j \in \epsilon(i)}$ and (2) a weighted sum of cross products between two differences $(X_j - X_i) \times (X_k - X_i)_{(j, k) \in \tau(i)}$. In Equation \ref{eq_15}, compared with multi-channel EGNNs in Section \ref{egnn}, our formula differs by the second term. More specifically, we use a function $\phi_t :\R ^ d \mapsto \R ^ {m \times m ^ \prime}$ to update the surface-aware messages $m_{ijk}$ and aggregate all the messages of the triangle faces that contain the vertex $i$. Finally, both features $X_i ^ {l+1}$ and $h_i ^ {l+1}$ are passed through a number of layers defined by the above Equations. 

\paragraph{Feature Initialization} 
Despite the existence of several preprocessing methods for extracting geometric features from mesh data, we propose a simple way to initialize invariant and multi-channel equivariant features for our MeshEGNN model. Notably, the model can be flexibly fit with different types of geometric features from mesh data. Each vertex $p$ in the mesh is augmented with invariant features, such as the average area $a_p \in \R$ collected from its adjacent faces as described in Section \ref{mesh}. Regarding the multi-channel equivariant feature, we stack the vertex coordinate $x_p \in \R ^ 3$ and the normal vector $n_p \in \R ^ 3$ to produce a multi-channel feature $X_p \in \R ^ {3 \times 2}$. Generally, 

\subsection{Analysis on Equivariance}
This section discusses the equivariance (invariance) properties of our model, including translations, rotations, and scale. First, as the surface's areas and normal vectors are invariant and equivariant under the SE(3)-transformations, our model is equivariant to translation and rotations (without reflections) {\color{blue}{Need proof ?}}. It is worth noting that the use of the cross product in Equation $\ref{eq_15}$ breaks 

For scale invariance, we normalize the initial position and normal vector of each vertex $i$ before proceeding to the proposed model:

  % def pos\_normalize(self, pos, batch):
  %       centroid = aggregate\_mean(pos, batch, batch.max()+1)[batch]
  %       pos = pos - centroid
  %       m = aggregate\_max(torch.sqrt(torch.sum(pos**2, axis=1)), batch, batch.max()+1)[batch]
  %       pos = pos / m.unsqueeze(-1)
  %       return pos



\paragraph{Scaling Invariance} 

%$(X ^ {l} _j - X_i ^ {l}) \times (X_k ^ {l} - X_i ^ {l})_{\all j, k \in \tau(i)}$.

% And the coordinate and the feature in the later layer $l+1$ is updated by:
% \begin{align*}
%     C_{\epsilon(i)}^{l+1} &= \sum_{j \in \epsilon(i)} (C_i^l - C_j^l) \phi_x (m_{ij}), \\
%     C_{\tau(i)}^{l+1} &= \sum_{j,k \in \tau(i)} [(C ^ {l} _j - C_i ^ {l}) \times (C_k ^ {l} - C_i ^ {l})] \phi_t(m_{ijk}), \\
%     C_i ^ {l+1} &= \phi_v(h_i ^ l) + \alpha C_{\epsilon(i)}^{l+1} + \beta C_{\tau(i)}^{l+1}, \\
%     h_i ^ {l+1} &= \phi_h(h_i ^ {l}, m_{\epsilon(i)}, m_{\tau(i)}).
% \end{align*}

% \textcolor{blue}{Todo: note that this breaks E(n) symmetry, instead being equivariant to SE(n)}

% \textcolor{blue}{I just rewrote the formula from Equations 11 to 16. In fact, we update the equivariant feature $X_i$ as in Equation 16. I guess normal vectors (cross product in Equation 15) are equivariant to reflections. Would you mind explaining why our formula breaks E(n) symmetry?  Thank you}. 


% \textcolor{blue}{A reflection would \emph{invert} the cross product, rather than just reflecting it. This isn't equivariant. 
% Imagine if the whole mesh was on the X-Y plane, and $X_{\tau(i)}^{l+1}$ is in the positive Z direction.
% If we apply a reflection to the mesh taking $(x, y, z) \mapsto (-x, y, z)$, then $X_{\tau(i)}^{l+1}$ would now be pointing in the negative Z direction.
% The resulting transformation of the output $X^{l+1}$ would then be $(x, y, z) \mapsto (-x, y, -z)$, which isn't the same as the transformation we applied to the input.}

% \textcolor{blue}{I get it now. Thanks for your explanation.}


\subsection{Hierarchical Interactions}
To facilitate long-range communications between nodes, after extracting information using MC-MeshEGNN layers, we employ a hierarchical structure that pools and unpools features at various resolutions. Our approach is inspired by the hierarchical structure interaction of PointNet++ \cite{qi2017pointnetplusplus} which  includes 2 main components - Pooling and Unpooling. In particular, the Pooling block - Equation \ref{eq_17} selects subset of vertices by Farthest Point Sampling $\text{FPS}$ algorithm and pooling the features from the neighbours of those chosen vertices. The neighbourhood of each vertex $\mathcal{N}(i^{L})$ is defined as a circular region around that vertex with a specific radius $r$.  In terms of the Unpooling block - Equation \ref{eq_18}, we merely interpolate the lower-leveled vertex features relied on the features of its $K$ nearest neighbours in the higher level and concatenate it with the original feature of that vertex $h_i^{L}$. The $L$ in the Equations \ref{eq_17} and \ref{eq_18} indicates the level of the vertices in the hierarchy.
\begin{align}
    P(h_i^{l}) &= \max_{j \in \mathcal{N}(i^{L})}(\phi(h_j)) \quad \text{where} 
    \quad i^{L} \in \text{FPS}(i^{L-1}) \label{eq_17} , \\
    U(h_i^{L}) &= \phi\bigg([h_i^{L}, \frac{\sum_{j\in\text{KNN}(i^{L}, i^{L+1})}\frac{1}{\|x_{ij}\|_2} h_j}{\sum_{j\in\text{KNN}(i^{L}, i^{L+1})} \frac{1}{\|x_{ij}\|_2}}]\bigg) \label{eq_18}. 
\end{align}

% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=0.8\linewidth]{iclr2024/visualization/update.png}
%   \caption{\label{fig:model} Draft}
% \end{figure}



% \begin{figure}[h!]
%   \centering
%   \includegraphics[width=1.\linewidth]{iclr2024/visualization/draft.png}
%   \caption{\label{fig:update} Information Update}
% \end{figure}
% % {\color{blue} face pooling ? Need to do}

% % {\color{blue}
% % $X = \frac{x -mean(x)}{max(\|x -mean(x)\|_2)}$ \\}

% % {\color{blue}
% % $N = \frac{n}{\|n\|_2} - mean(\frac{n}{\|n\|_2})$
% % }

==> old/5.experiments.tex <==
In this section, we evaluate our model by two types of pipelines including equivariant and non-equivariant (normal) datasets. Each setting covers both node-level and graph-level classification. Regarding the input of our experiments, we use vertex coordinates and normal vectors in equivariant datasets, while in non-equivariant we additionally pre-compute HKS \cite{Sun2009ACA} following recent pipeline such as \cite{diffusionnet}, \cite{laplacian2mesh}, and \cite{meshmlp}. Moreover, since our model is designed to be equivariant with E(n) transformations and invariant to scaling, we use no augmentations when training our MeshEGNN.

\subsection{Equivariant Mesh Datasets}
Equivariant mesh datasets comprise TOSCA \cite{tosca} and FAUST \cite{faust}.:
\begin{itemize}
    \item TOSCA is a 9-class mesh dataset with varying nodes and edges in each mesh. The total samples of this dataset is 80, where 63 meshes are used for training and 17 meshes are used for evaluation . The main task of this dataset is to classify input mesh with correct labels.
    \item FAUST includes 100 samples of 3-dimensional human meshes with 6890 vertices each. In each mesh, the vertices are numbered so that the vertices correspond to the same “location” on the human meshes are labelled with the same number. This is a segmentation task where the model needs to predict the labels for all vertices in the mesh.
\end{itemize}

\begin{table}[h!]
\caption{Means and standard deviations over 5 seeds of the segmentation accuracy on the FAUST dataset. No data augmentation is applied during training.}
\begin{center}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c c c c c c c}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Initial Features} & \multicolumn{5}{c}{Accuracy (\%)} \\
\cmidrule(l r){3-7}
&  & Train & Test & Gauge & Rot-Tr-Scale & Perm \\
\midrule
\multirow{4}{*}{GEM-CNN \cite{gemcnn}} & XYZ & $99.42(0.15)$ & $97.92(0.30)$ & $96.90(0.25)$ & $2.14(1.49)$ & $97.92(0.30)$ \\
 & GET & $99.42(0.15)$ & $98.03(0.17)$ & $97.15(0.39)$ & $1.47(1.60)$ & $98.03(0.17)$ \\
 & RELTAN $[0.7]$ & $99.69(0.05)$ & $98.62(0.06)$ & $98.04(0.12)$ & $98.62(0.06)$ & $98.62(0.06)$ \\
 & RELTAN $[0.5,0.7]$ & $99.70(0.09)$ & $98.64(0.22)$ & $97.99(0.18)$ & $98.64(0.22)$ & $98.64(0.22)$ \\
\midrule
\multirow{4}{*}{EMAN \cite{eman}} & XYZ & $99.62(0.09)$ & $98.46(0.15)$ & $97.26(0.34)$ & $0.02(0.00)$ & $98.46(0.15)$ \\
 & GET & $99.60(0.08)$ & $98.43(0.17)$ & $97.32(0.46)$ & $0.02(0.00)$ & $98.43(0.17)$ \\
 & RELTAN $[0.7]$ & $99.27(1.01)$ & $98.13(1.19)$ & $97.44(1.26)$ & $98.13(1.19)$ & $98.13(1.19)$ \\
 & $\operatorname{RELTAN}[0.5,0.7]$ & $99.68(0.00)$ & $98.66(0.07)$ & $98.41(0.25)$ & $98.66(0.07)$ & $98.66(0.07)$ \\
\midrule
EGNN (baseline) & XYZ & $99.70(0.02)$ & $99.50(0.02)$ & $99.50(0.02)$ & $99.50(0.02)$ & $99.50(0.02)$ \\
EGNN + MC (baseline) & XYZ + Normal & $99.80(0.02)$ & $99.76(0.01)$ & $99.76(0.01)$ & $99.76(0.01)$ & $99.76(0.01)$ \\
\midrule
MeshEGNN (ours) & XYZ & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00) $ & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$\\
MeshEGNN (ours) + MC & XYZ + Normal & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$& $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$\\
\bottomrule
\end{tabular}}
\end{center}
\end{table}

\begin{table}[h!]
\caption{Means and standard deviations over 5 seeds of the segmentation accuracy on the TOSCA dataset. No data augmentation is applied during training.}
\begin{center}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{c c c c c c}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Initial Features}  & \multicolumn{4}{c}{Accuracy (\%)} \\
\cmidrule(l r){3-6}
&  & Train & Test & Gauge & Rot-Tr-Scale \\
\midrule
\multirow{4}{*}{GEM-CNN \cite{gemcnn}} & XYZ & $9 7 . 7 8(2.41)$ & $82.35(5.88)$ & $82.35(5.88)$ & $1 2 . 9 4(2.63)$ \\
 & GET & $90.79(2.84)$ & $82.35(9.30)$ & $82.35(9.30)$ & $1 7 . 6 5(7.20)$ \\
 & ReLTAN[0.7] & $93.97(4.26)$ & $91.76(6.71)$ & $91.76(6.71)$ & $91.76(6.71)$ \\
 & RELTAN[0.5, 0.7] & $90.16(8.43)$ & $89.41(14.65)$ & $89.41(14.65)$ & $89.41(14.65)$ \\
\midrule
\multirow{4}{*}{EMAN \cite{eman}} & XYZ & $47.30(4.55)$ & $42.35(20.55)$ & $44.71(18.88)$ & $12.94(2.63)$ \\
 & GET & $44.13(7.39)$ & $42.35(11.31)$ & $41.18(9.30)$ & $1 0 . 5 9(2.63)$ \\
 & ReLTAN[0.7] & $92.70(4.14)$ & $94.12(4.16)$ & $94.12(4.16)$ & $94.12(4.16)$ \\
 & ReLTAn[0.5, 0.7] & $97.46(4.14)$ & $9 8 . 8 2(2.63)$ & $98.82(2.63)$ & $9 8 . 8 2(2.63)$ \\
\midrule
EGNN (baseline) & XYZ & $96.82(0.11)$ & $95.23(0.11)$ & $95.23(0.11)$ & $95.23(0.11)$ \\
EGNN + MC (baseline) & XYZ + Normal & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$& $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$ \\
\midrule
MeshEGNN (ours) & XYZ & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$ \\
MeshEGNN + MC (ours) & XYZ + Normal & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$ & $\mathbf{100.00}(0.00)$ \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}

\begin{table}[h!]
\caption{Runtime + Memory}
\begin{center}
\begin{tabular}{c c c c c}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{FAUST} & \multicolumn{2}{c}{TOSCA}\\
\cmidrule(l r){2-3} \cmidrule(l r){4-5}
 & Runtime & Memory & Runtime & Memory \\
\midrule
GEM-CNN \cite{gemcnn} & 21s & 2.2GB & 60s & 4.3GB \\
EMAN \cite{eman} & 53s & 2.2GB & 120s & 6.6GB \\
\midrule
EGNN (baseline) & 1s & 2.1GB & 2s & 2.7GB \\
EGNN + MC (baseline) & 1.5s & 2.1GB & 3s & 2.7GB \\
\midrule
MeshEGNN (ours) & 3s & 2.1GB & 7s & 3.6GB \\
MeshEGNN + MC (ours) & 4s & 2.1GB & 11s & 3.9GB \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

\subsection{Mesh Datasets}
In terms of normal datasets, we test the performance of our model on SHRED and Human Body Segmentation:
\begin{itemize}
    \item SHREC-11  \cite{shrec11}  contains 30 different classes (20 samples per class).
    There are 2 settings commonly followed to evaluate the model on this dataset, which are  10-10 and 16-4 train-test split.
    \item Human Body Segmentation has 370 meshes for training and 18 meshes for testing, which collected from Adobe Fuse \cite{Adobe16}, FAUST \cite{faust}, MIT \cite{Vlasic2008ArticulatedMA}, SCAPE \cite{Klokov2017EscapeFC}, and SHREC07 \cite{giorgi2007shape}. Thereafter all the meshes are labeled into 8 parts by \cite{giorgi2007shape}.
\end{itemize}



\begin{table}[h!]
\begin{center}
\caption{SHRED - cls}
\vspace{5pt}
\begin{tabular}{l c c c c}
\toprule
Method & Runtime & Memory & Split-16 & Split-10\\
\midrule
GWCNN \cite{gwcnn} & --- & --- & $96.6 \%$ & $90.3 \%$ \\
MeshCNN \cite{meshcnn} & 50s & 1.2GB & $98.6 \%$ & $91.0 \%$\\
PD-MeshNet \cite{Milano20NeurIPS-PDMeshNet} & --- & --- & $99.7 \%$ & $99.1 \%$ \\
MeshWalker\cite{lahav2020meshwalker} & --- & --- & $98.6 \%$ & $97.1 \%$ \\
SubdivNet \cite{DBLP:journals/tog/HuLGCHMM22} & 25s & 0.9GB & $99.9 \%$ & $99.5 \%$ \\
HodgeNet \cite{smirnov2021hodgenet} & --- & --- & $99.2 \%$ & $94.7 \%$ \\
DiffusionNet\cite{diffusionnet} & 16s & 1.0GB & --- & $99.5 \%$ \\
Laplacian2Mesh \cite{laplacian2mesh}& 30s & 2.8GB & $\mathbf{100}\% $ &  $\mathbf{100}\%$\\
Mesh-MLP \cite{meshmlp}& --- & --- & $\mathbf{100}\%$ & $\underline{99.7}\%$\\
\midrule
EGNN (baseline) & 11s & 0.8GB &  $99.1\%$ & $96.3\%$ \\
EGNN + MC (baseline)& 11s & 0.8GB & $100\%$ & $99.3\%$  \\
\midrule
MeshEGNN (ours) & 24s & 1.1GB & $\mathbf{100}\%$ & $97.3\%$\\
MeshEGNN + MC (ours) & 25s & 1.1GB & $\mathbf{100}\%$ & $\underline{99.7}\%$\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

\begin{table}[h!]
\caption{HUMAN - seg}
\vspace{5pt}
\begin{center}
\begin{tabular}{l c c c c}
\hline
Method & Input & Runtime & Memory & Accuracy \\
\hline
PointNet \cite{qi2016pointnet} & point cloud & 12s & 1.2GB & $74.7 \%$ \\
PointNet++\cite{qi2017pointnetplusplus}& point cloud & 10s & 0.9GB & $82.3 \%$ \\
\hline
MeshCNN \cite{meshcnn} & mesh & 137s & 1.4GB & $85.4 \%$ \\
PD-MeshNet \cite{Milano20NeurIPS-PDMeshNet} & mesh & --- & --- & $85.6 \%$ \\
SubdivNet \cite{DBLP:journals/tog/HuLGCHMM22} & mesh & 100s & 1.3GB & $91.7\%$\\ 
DiffusionNet \cite{diffusionnet} & mesh & 16s & 2.0GB & $90.3\%$ \\ 
HodgeNet \cite{smirnov2021hodgenet} & mesh & --- & --- & $85.0 \%$ \\
Laplacian2Mesh \cite{laplacian2mesh} & mesh & 70s & 4.8GB & $88.6 \%$ \\
Mesh-MLP \cite{meshmlp} & mesh & --- & --- & $88.8\%$ \\
\hline
EGNN (baseline) & graph & 10s & 0.8GB & $80.6\%$ \\
EGNN+MC (baseline) & graph & 11s & 0.8GB & $82.7\%$  \\
EGNN+MC+Hier (baseline) & graph & 16s & 0.9GB & $87.2\%$  \\
\hline
MeshEGNN (ours) & mesh & 18s & 0.9GB & $81.0\%$ \\
MeshEGNN+MC (ours) & mesh & 20s & 0.9GB & $83.5\%$ \\
MeshEGNN+MC+Hier (ours) & mesh & 26s & 1.0GB & 88.7\%\\
\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Ablation Study}

\begin{table}[h!]
\begin{center}
\centering
\caption{\label{tab:ab_cluster_hierarchy} Ablation study on Layers, Hierarchy, Channels}
\begin{tabular}{c c c c c c} 

\toprule
\textbf{Layers} & \textbf{Accuracy} & \textbf{Hierarchy}  & \textbf{Accuracy} & \textbf{Channels} & \textbf{Accuracy}\\
\cmidrule(l r){1-2} \cmidrule(l r){3-4} \cmidrule(l r){5-6}
2  & 87.5 & 2  & 88.2 & 2 & 88.7\\ 
3  & 88.7 & 3  & 88.7 & 4 & 86.3\\ 
4  & 88.0 & 4  & 87.6  & 8 & 88.2\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

